Learning Compositional Neural Programs for Continuous Control

We propose a novel solution to challenging sparse-reward, continuous control problems that require hierarchical planning at multiple levels of abstraction. Our solution, dubbed AlphaNPI-X, involves three separate stages of learning. First, we use off-policy reinforcement learning algorithms with experience replay to learn a set of atomic goal-conditioned policies, which can be easily repurposed for many tasks. Second, we learn self-models describing the effect of the atomic policies on the environment. Third, the self-models are harnessed to learn recursive compositional programs with multiple levels of abstraction. The key insight is that the self-models enable planning by imagination, obviating the need for interaction with the world when learning higher-level compositional programs. To accomplish the third stage of learning, we extend the AlphaNPI algorithm, which applies AlphaZero to learn recursive neural programmer-interpreters. We empirically show that AlphaNPI-X can effectively learn to tackle challenging sparse manipulation tasks, such as stacking multiple blocks, where powerful model-free baselines fail.

==> algo.tex <==
\begin{algorithm}[!ht]
\SetAlgorithmName{Algorithm}{}
\KwData{}
{\small
\textbf{Given}: 
\begin{itemize}
    \item an off-policy algorithm $\mathbb{A}$ \Comment{e.g. TD3, SAC}
    \item a strategy $\mathbb{S}$ for sampling goals for replay
    \item an initial goal sampling strategy $\mathbb{G}$
\end{itemize}

Initialize $\mathbb{A}$

Initialize replay buffer $R$ and $R^{'}$

\For{\emph{episode = 1}, \dots, M}{
        Sample a goal $g$ according to $\mathbb{G}$ and an initial state $s_0$
        
        \While{\emph{$a_t$ != Stop}}{
        	Sample an action $a_t$ using the behavioral policy from $\mathbb{A}$
        	
        	Execute the action $a_t$ and observe a new state $e_{t+1}$ and reward $r_t$
        	
        	Store the transition $(e_t, a_t, r_t, e_{t+1}, g)$ in $R$
        	
    	}
    	Check if final episode state $s_T$ verifies a motion program post-condition
    	
    	If program $i$ post-condition are verified, store the transitions $(e_t, a_t, r_t, e_{t+1}, i)$ in $R^{'}$
    	
    	Sample set of additional goals for replay according to $\mathbb{S}$ and store in buffer \Comment{HER}
    	
    	\For{\emph{training\_iteration = 1}, \dots, N}{
    	    Sample a minibatch B from the replay buffer $R$
    	    
    	    Perform one backward pass on the motion module using $\mathbb{A}$ and minibatch B
    	    
    	    If $R^{'}$ is not empty, sample a minibatch $B^{'}$ from $R^{'}$
    	    
    	    Perform one backward pass on the motion + program module using $\mathbb{A}$ and minibatch $B^{'}$
    	}
       
    } 

}
\caption{AlphaNPI motion module training algorithm}
\label{alg:tree_search}
\end{algorithm}

==> litterature_review.tex <==
@article{stack-4-cubes,
  author    = {John B. Lanier and
               Stephen McAleer and
               Pierre Baldi},
  title     = {Curiosity-Driven Multi-Criteria Hindsight Experience Replay},
  journal   = {CoRR},
  volume    = {abs/1906.03710},
  year      = {2019},
  url       = {http://arxiv.org/abs/1906.03710},
  archivePrefix = {arXiv},
  eprint    = {1906.03710},
  timestamp = {Fri, 14 Jun 2019 09:38:24 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1906-03710},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{option-critic,
  author    = {Pierre{-}Luc Bacon and
               Jean Harb and
               Doina Precup},
  title     = {The Option-Critic Architecture},
  journal   = {CoRR},
  volume    = {abs/1609.05140},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.05140},
  archivePrefix = {arXiv},
  eprint    = {1609.05140},
  timestamp = {Mon, 13 Aug 2018 16:48:17 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/BaconHP16},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{data-efficient-hrl,
  author    = {Ofir Nachum and
               Shixiang Gu and
               Honglak Lee and
               Sergey Levine},
  title     = {Data-Efficient Hierarchical Reinforcement Learning},
  journal   = {CoRR},
  volume    = {abs/1805.08296},
  year      = {2018},
  url       = {http://arxiv.org/abs/1805.08296},
  archivePrefix = {arXiv},
  eprint    = {1805.08296},
  timestamp = {Mon, 13 Aug 2018 16:46:14 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1805-08296},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{sac-x,
  author    = {Martin A. Riedmiller and
               Roland Hafner and
               Thomas Lampe and
               Michael Neunert and
               Jonas Degrave and
               Tom Van de Wiele and
               Volodymyr Mnih and
               Nicolas Heess and
               Jost Tobias Springenberg},
  title     = {Learning by Playing - Solving Sparse Reward Tasks from Scratch},
  journal   = {CoRR},
  volume    = {abs/1802.10567},
  year      = {2018},
  url       = {http://arxiv.org/abs/1802.10567},
  archivePrefix = {arXiv},
  eprint    = {1802.10567},
  timestamp = {Mon, 13 Aug 2018 16:47:06 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1802-10567},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{curious,
  author    = {C{\'{e}}dric Colas and
               Pierre Fournier and
               Olivier Sigaud and
               Pierre{-}Yves Oudeyer},
  title     = {{CURIOUS:} Intrinsically Motivated Multi-Task, Multi-Goal Reinforcement
               Learning},
  journal   = {CoRR},
  volume    = {abs/1810.06284},
  year      = {2018},
  url       = {http://arxiv.org/abs/1810.06284},
  archivePrefix = {arXiv},
  eprint    = {1810.06284},
  timestamp = {Tue, 30 Oct 2018 20:39:56 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1810-06284},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{language-abstraction-hrl,
  author    = {Yiding Jiang and
               Shixiang Gu and
               Kevin Murphy and
               Chelsea Finn},
  title     = {Language as an Abstraction for Hierarchical Deep Reinforcement Learning},
  journal   = {CoRR},
  volume    = {abs/1906.07343},
  year      = {2019},
  url       = {http://arxiv.org/abs/1906.07343},
  archivePrefix = {arXiv},
  eprint    = {1906.07343},
  timestamp = {Mon, 24 Jun 2019 17:28:45 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1906-07343},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{ther,
    title={Self-Educated Language Agent With Hindsight Experience Replay For Instruction Following},
    author={Geoffrey Cideron and Mathieu Seurin and Florian Strub and Olivier Pietquin},
    year={2019},
    eprint={1910.09451},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}



==> tables/alphanpi_lpcurr_performance.tex <==
\begin{table}[H]
\label{table:alphanpi_final_perf}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccc}
\toprule
\textbf{Program} & \textbf{No Planning}  & \textbf{Planning without MPC} & \textbf{Planning with MPC}\\
\midrule
{\sc Clean\_Table} & 0.02 & 0.03 & 0.18\\
{\sc Clean\_And\_Stack} & 0.08 & 0.07 & 0.44\\
{\sc Stack\_All\_Blocks} & 0.00 & 0.25 & 0.42\\
{\sc Stack\_All\_To\_Zone} & 0.80 & 0.92 & 0.92\\
{\sc Move\_All\_To\_Zone} & 0.68 & 0.95 & 0.95\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{Our trained \anx performance. We compare \anx when planning in MPC style, without MPC and when relying on its neural network alone, without tree search. Each program is executed 100 times for each configuration. For programs with arguments, the performance is averaged over all possible arguments combinations.}
\vskip -0.1in
\end{table}

==> tables/programs_conditions_table.tex <==
\begin{table*}[t]
\label{table:program_library_preconds}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lll}
\toprule
\textbf{program} & \textbf{pre-condition}\\
\midrule
\vspace{-0.2cm}
{\sc Stack} & \Longunderstack[l]{\noindent The block to be moved might be moved without moving other objects\\ and there is free space above the block to stack on \\}\\
\vspace{-0.2cm}
{\sc Move\_To\_Zone} & \Longunderstack[l]{\noindent The block to be moved might be moved without moving other objects\\ and is not already on the target zone \\}\\
\hline
{\sc Stack\_All\_Blocks} & No precondition\\
{\sc Stack\_All\_To\_Zone} & No precondition\\
{\sc Move\_All\_To\_Zone} & No precondition\\
\hline
{\sc Clean\_Table} & No precondition \\
{\sc Clean\_And\_Stack} & No precondition \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{Programs library preconditions.}
\vskip -0.1in
\end{table*}


\begin{table*}[t]
\label{table:program_library_postconds}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lll}
\toprule
\textbf{program} & \textbf{post-condition}\\
\midrule
{\sc Stack} & The block to be moved has been placed above the block to stack on.\\
{\sc Move\_To\_Zone} & The block has been moved in the target zone.\\
\hline
{\sc Stack\_All\_Blocks} & All the blocks have been stacked together in any arbitrary order.\\
{\sc Stack\_All\_To\_Zone} & Both blocks have been stacked in any order in the target zone.\\
{\sc Move\_All\_To\_Zone} & Both blocks have been moved to the target zone.\\
\hline
{\sc Clean\_Table} & For each colour, both blocks have been moved to the correct zone. \\
{\sc Clean\_And\_Stack} & \Longunderstack[l]{\noindent For each colour, both blocks have been stacked\\ in any order in the correct zone.}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{Programs library postconditions.}
\vskip -0.1in
\end{table*}

==> tables/programs_descriptions.tex <==
\begin{table*}[t]
\label{table:program_library}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{ll}
\toprule
\textbf{program} & \textbf{description}\\
\midrule
{\sc Stack} & Stack a block on another block.\\
{\sc Move\_To\_Zone} & Move a block to a color zone.\\
\hline
{\sc Stack\_All\_Blocks} & Stack all blocks together.\\
{\sc Stack\_All\_To\_Zone} & Stack blocks of the same color in a zone.\\
{\sc Move\_All\_To\_Zone} & Move blocks of the same color to a zone.\\
\hline
{\sc Clean\_Table} & Move all blocks to their color zone.\\
{\sc Clean\_And\_Stack} & Stack blocks of the same color in the corresponding zone.\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{Descriptions of the fetch environment programs.}
\vskip -0.1in
\end{table*}
